Weisfeiler-Lehman goes Dynamic: An Analysis of the Expressive Power of Graph Neural Networks for Attributed and Dynamic Graphs

Graph Neural Networks (GNNs) are a large class of relational models for graph processing. Recent theoretical studies on the expressive power of GNNs have focused on two issues. On the one hand, it has been proven that GNNs are as powerful as the Weisfeiler-Lehman test (1-WL) in their ability to distinguish graphs. Moreover, it has been shown that the equivalence enforced by 1-WL equals unfolding equivalence. On the other hand, GNNs turned out to be universal approximators on graphs modulo the constraints enforced by 1-WL/unfolding equivalence. However, these results only apply to Static Attributed Undirected Homogeneous Graphs (SAUHG) with node attributes. In contrast, real-life applications often involve a much larger variety of graph types. In this paper, we conduct a theoretical analysis of the expressive power of GNNs for two other graph domains that are particularly interesting in practical applications, namely dynamic graphs and SAUGHs with edge attributes. Dynamic graphs are widely used in modern applications; hence, the study of the expressive capability of GNNs in this domain is essential for practical reasons and, in addition, it requires a new analyzing approach due to the difference in the architecture of dynamic GNNs compared to static ones. On the other hand, the examination of SAUHGs is of particular relevance since they act as a standard form for all graph types: it has been shown that all graph types can be transformed without loss of information to SAUHGs with both attributes on nodes and edges. This paper considers generic GNN models and appropriate 1-WL tests for those domains. Then, the known results on the expressive power of GNNs are extended to the mentioned domains: it is proven that GNNs have the same capability as the 1-WL test, the 1-WL equivalence equals unfolding equivalence and that GNNs are universal approximators modulo 1-WL/unfolding equivalence.

==> sections/limitations-WL-tests.tex <==
\section{Weisfeiler-Lehmann Hierarchy}\label{section_WL_hierarchy}

In this section we aim to position the attributed WL tests into the Weisfeiler Lehmann Hierarchy.

\begin{Thm}\label{thm_1WL_vs_attrib_1WL}
1-WL test $\subsetneq$ attributed 1-WL test
\end{Thm}

%\textcolor{orange}{I think  you proved  a stronger result of what you inserted in the theorem. Actually, 
%attributed 1-WL test uses edge/node features  and it is obvious that if the
%difference between two graphs is due to such an information 1-WL test cannot get it. 
%Consider two  nodes linked by an edge. The feature of the edge allows to distinguish any graph of this type.
%Thus, 1-WL test $\subsetneq$ attributed 1-WL test is obvious. On the other hand, I think that  the result is more
%interesting because the inequality holds for graphs that are not isomorphic (without considering features). 
%Figure \ref{fig_limitations_dynamic_WL}a,b shows an example of a non isomorphic graph for which the inequality holds. 
%}

%\textcolor{orange}{I think the result is interesting. Verify whether it is already available in literature,
%even if I understand it is not easy to check.}

\begin{proof} First we show that 1-WL test is a subset of the attributed 1-WL test and then we give a counter example for them being equal. 
\begin{itemize}
    \item[$\subset$] Due to Thm.~\ref{ue=wl} the WL test is equivalent to the unfolding tree equivalence. Therefore, the equality of the attributed trees leads to an equality in those trees underlying tree structure,  i.e., if two graphs are attributed-wise unfolding equivalent they are unfolding equivalent. Hence, if two graphs are attributed-wise WL equivalent, they are 1-WL equivalent.
    \item[$\neq$] In Fig.~\ref{fig_limitations_dynamic_WL} one can see that the attributed WL test can distinguish the first and last graph (graphs a and c), while the 1-WL test fails.
\end{itemize}
\end{proof}


\begin{figure}[h]
    \centering
    \includegraphics[width=\textwidth]{figures/limitation_dyn_WL.pdf}
    \caption{The graphs a) and b) are falsely recognized as 1-WL and attributed 1-WL isomorphic; same holds for the 3-WL and 3-AWL. The graphs b) and c) are falsely recognized isomprohic just by the 1-WL/3-WL test while the 1-AWL/3-AWL test correctly recognizes both graphs as non isomorphic. The same result holds for the graphs b) and c) for 1-WL and 1-AWL while 3-WL and 3-AWL can distinguish both. The 1-WL and 3-WL equivalences on the graphs from a) and b) and a) and c) without attributes are taken from \cite[§3.1]{sato2020survey}}.
    \label{fig_limitations_dynamic_WL}
\end{figure}


\begin{Cor}
2-WL test $\subsetneq$ attributed 1-WL test
\end{Cor}
\begin{proof}
As stated in \cite[§3.5, Cor.~3.5.8]{grohe2017descriptive}, 1-WL test and 2-WL test are equivalent.
\end{proof}
%\textcolor{orange}{I could not find where it is states that  1-WL test and 2-WL test are equivalent. Could you
%tell me where is?}\textcolor{red}{We find the actual paper in which it is proven...The statement says that "two graphs are equivalent by the colouring algorithm (i.e. 1-WL test) iff they are equivalent by the 2-WL test. }


\begin{Cor}
k-WL test $\subsetneq$ attributed k-WL test.
\end{Cor}
\begin{proof}
Follows analogously from the proof of Thm.~\ref{thm_1WL_vs_attrib_1WL}.
\end{proof}
\textcolor{orange}{Here, we have the same problem of the previous theorem. The inequality is obvious, but can we prove for non isomorphic graphs? }

\begin{Cor}
The dynamic k-WL test $\subseteq$ dynamic (k+1)-WL test.
\end{Cor}
\begin{proof}
Follows immediately from the static Weisfeiler-Lehmann Hierarchy.
\end{proof}
\textcolor{orange}{}
\begin{Thm}
The 3-WL test and the attributed 1-WL test cannot be compared regarding to the Weisfeiler Lehmann Hierarchy.
\end{Thm}

\begin{Thm}
Let $G_1 = (\mathcal{V}_1, \mathcal{E}_1, \alpha_1)$ and $G_2 = (\mathcal{V}_2, \mathcal{E}_2, \alpha_2)$ be to graphs with $G_1 \nsim_{WL} G_2$. Then there exists at least one $\omega_1, \omega_2$ such that $G_1 \nsim_{AWL} G_2$. 
\end{Thm}

\begin{proof}
THATS SO TRIVIAL, because I can just set $\omega_i(\mathcal{E}) \mapsto x$ for a fix but arbitrary $x \in B$ , or not?
\end{proof}

\begin{proof}
In Fig.~\ref{fig_limitations_dynamic_WL} one can see that the 3-WL test can distinguish the graphs a) and b) but the attributed 1-WL test cannot. However, the 3-WL test cannot distinguish the graphs b) and c) while the attributed 1-WL test can. 
\end{proof}

\begin{paragraph}{Remark.} Another comparison we haven't talked about yet is between the dynamic 1-WL test and the attributed 1-WL test. In fact, these two tests refer to mathematically different objects. The dynamic 1-WL test is defined only on dynamic nodes of dynamic graphs, while the attributed 1-WL test is defined on static nodes of static graphs. 
Therefore, they cannot be related with respect to the Weisfeiler-Lehmann hierarchy. In other words, this hierarchy is only a partial order and not a total order when all possible WL tests and extensions are considered. 
\end{paragraph}



